Convergence of the harmonic balance method for smooth Hilbert space valued differential-algebraic equations

We analyze the convergence of the harmonic balance method for computing isolated periodic solutions of a large class of continuously differentiable Hilbert space valued differential-algebraic equations (DAEs). We establish asymptotic convergence estimates for (i) the approximate periodic solution in terms of the number of approximated harmonics and (ii) the inexact Newton method used to compute the approximate Fourier coefficients. The convergence estimates are deter-mined by the rate of convergence of the Fourier series of the exact solution and the structure of the DAE. Both the case that the period is known and unknown are analyzed, where in the latter case we require enforcing an appropriately defined phase condition. The theoretical results are illustrated with several numerical experiments from circuit modeling and structural dynamics.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk --shell-escape -pdf \"$_[0]\"" );
    }
}

==> proofofunknown.tex <==
\begin{comment}
\begin{proof}
The proof is an application of Theorem \ref{thm:inexactNK}, analogous to the proof of Theorem \ref{thm:known}.  Assume that $N \geq N_1$ and $(x_0^N,\tau_0^N) \in \mc{B}((\alpha_N,T),\xi_N)$ where $\xi_N \leq \delta_{N,\sigma}$.  It then follows that:
$$x_0^N \in \mc{B}(\alpha_N,\delta_{N,\sigma}), \quad |\tau_0^N-T| \leq \xi_N \leq \delta.$$
Lemma \ref{lem:DxRhat}, Estimate \eqref{eq:DxRhat.1} therefore implies that:
$$\|[D \hat R_N(x_0^N,\tau_0^N)]^{-1}\| \leq K_L.$$  
We first estimate $\|[D \hat R_N(x_0^N,\tau_0^N)]^{-1} ( D\hat R_N(z,w) - D\hat R_N(y,s))\|$. If $\|(z,w)-(y,s)\| \leq \delta_N$, then:
\begin{align*}
\|[& D \hat R_N(x_0^N,\tau_0^N)]^{-1} ( D\hat R_N(z) - D\hat R_N(y))\| \\
& \leq \|[D\hat R_N(x_0^N,\tau_0^N)]^{-1}\| \cdot \|D \hat R_N(y,s)-D \hat R_N(z,w)\|\\
& \leq K_L \|D \hat R_N(y,s)-D \hat R_N(z,w)\| && (\|[D \hat R_N(x_0^N,\tau_0^N)]^{-1}\| \leq K_L)\\
& \leq K_L L_2 N^{M_2}\|(z,w)-(y,s)\| && \text{(Lemma \ref{lem:DxxRlem}, Estimate \eqref{eq:DxxRlem.2b})}\\
& \leq \underbrace{\text{max}\{K_L L_2, 2\delta^{-1}(2\pi)^k \}}_{\equiv \hat L_2}(N+1)^{M_2 + \rho_2}\|(z,w)-(y,s)\|.
\end{align*}
We define $L_N > 0$ as:
\begin{equation}\label{eq:Ldef}
L_N = \hat{L}_2(N+1)^{M_2 +\rho_2}.
\end{equation} 
By construction $L_N^{-1} \leq \delta_N$, since $N \geq N_1$.  Therefore $\mc{B}((\alpha_N,T),L_N^{-1}) \subseteq \mc{B}((\alpha_N,T),\delta_N)$ so:
\begin{equation}\label{eq:unknown.NK1}
\|[D \hat R_N(x_0^N,\tau_0^N)]^{-1}(D \hat R_N(z,w) - D \hat R_N(y,s))\| \leq L_N \|z-y\|,  \quad \forall (y,s),(z,w) \in \mc{B}((\alpha_N,T),L_N^{-1}).
\end{equation}
We next estimate $\|[D \hat R_N(x_0^N,\tau_0^N)]^{-1} \hat R_N(x_0^N,\tau_0^N)\|$:
\begin{align*}
\|[D \hat R_N(x_0^N,\tau_0^N)]^{-1} \hat R_N(x_0^N,\tau_0^N)\|& \leq \|[D \hat R_N(x_0^N,\tau_0^N)]^{-1}\| \cdot \|\hat R_N(x_0^N,\tau_0^N)\| \\
& \leq K_L \|\hat R_N(x_0^N,\tau_0^N)\| && (\|[D \hat R_N(x_0^N,\tau_0^N)]^{-1}\|\leq K_L) \\
& =  K_L (\|R_N(x_0^N,\tau_0^N)\|^2 + |\sigma_N(x_0^N)|^2)^{1/2} \\ 
& \leq  K_L (\|R_N(x_0^N,\tau_0^N)\| + |\sigma_N(x_0^N)|) \\ 
& \leq  K_L (\|\mc{F}_N(x_0^N,\tau_0^N)\|_{L^2} + |\sigma_N(x_0^N)|). && \text{(Lemma \ref{lem:DxxRlem}, Estimate \eqref{eq:DxxRlem.1})}
\end{align*}
Since $\|x_0^N - \alpha_N\| \leq \xi_N \leq \delta_N = \zeta_N(\delta)$, $N \geq N_1$, and $\delta(\mc{A}) \in (0,\text{min}\{\mc{A},1\}]$, Lemma \ref{lem:Qlem2} implies: 
$$\|Q_N(x_0^N) -p\|_{H^k} \leq \delta(\mc{A}) \leq 1.$$
Since $|\tau_0^N-T| \leq \delta_N \leq T/2$ also holds, Estimates \eqref{eq:defJ1J2} and \eqref{eq:defJsigma} then imply  that:
$$\|\mc{F}_N(x_0^N,\tau_0^N)\|_{L^2} + |\sigma_N(x)| \leq (J_1+ J_{\sigma})\|Q_N(x_0^N) - p\|_{H^k} + J_2|\tau_0^N-T|.$$
Therefore:
$$\|[D \hat R_N(x_0^N,\tau_0^N)]^{-1} \hat R_N(x_0^N,\tau_0^N)\|  & \leq  K_L(J_1 +  J_{\sigma}) \|Q_N(x_0^N) - p\|_{H^k} + K_L J_2|\tau_0^N-T|.$$
This together with Estimate \eqref{eq:Qpbound} implies:
\begin{equation}\label{eq:unknown.NK2}
\|[ D & \hat R_N(x_0^N,\tau_0^N)]^{-1} \hat R_N(x_0^N,\tau_0^N)\| \leq \beta_N(x_0^N,\tau_0^N)
\end{equation}
where
\begin{equation}\label{eq:unknown.beta}
\beta_N(x_0^N,\tau_0^N) :=  \sqrt{2} K_L (J_1 + J_2 + J_{\sigma})\Bigr(\sum_{j=0}^{k} (2\pi N)^j\Bigr)\|(x_0^N,\tau_0^N) - (\alpha_N,T)\| + K_L (J_{1} + J_{\sigma}) K_p(N).
\end{equation}
We then have:
\begin{align*}
\beta_N(x_0^N) L_N & \leq K_L (J_{1} + J_{\sigma})\hat L_2 (2\pi)^k (N+1)^{M_2 + \rho_2} K_p(N)\\
& \quad \quad + \sqrt{2} K_L( J_{1} + J_2 + J_{\sigma}) \hat L_2 (N+1)^{M_2 + \rho_2}\Bigr( \sum_{j=0}^{k}(2\pi N)^j
\Bigr)\|(x_0^N,\tau_0^N) - (\alpha_N,T)\| 
\end{align*}
Estimate \eqref{eq:unknown.0} implies there exists $N_* \geq N_1$ such that:
$$ K_L (J_{1}+ J_{\sigma})\hat L_2 (2\pi)^k (N+1)^{M_2+ \rho_2}K_p(N) \leq \ve/2, \quad N \geq N_*.$$
Let $C> 0$ be defined by:
$$C = \text{min}\{(2\sqrt{2} K_L (J_1 + J_2 + J_{\sigma}) \hat L_2^{-1} \ve,\hat L_2^{-1}/2\}.$$
If $N$ and $\xi_N$ satisfy 
\begin{equation}\label{eq:unknown.asp}
N \geq N_*, \quad \xi_N \leq \text{min}\left\{\delta_N,C(N+1)^{-(M_2+\rho_2)}\Bigr(\sum_{j=0}^{k}(2\pi N)^j\Bigr)^{-1}\right\},
\end{equation}
then 
\begin{equation}\label{eq:xnltnl}
\beta_N(x_0^N,\tau_0^N) L_N \leq \ve < 1/2, \quad \xi_N \leq L_N^{-1}/2.
\end{equation}
For the remainder of the proof, assume $N$ and $\xi_N$ satisfy the estimates in \eqref{eq:unknown.asp}.  Suppose that we solve $R_N(\cdot,\cdot) = 0$ using an inexact Newton method with initial guess $(x_0^N,\tau_0^N) \in \mc{B}((\alpha_N,T),\xi_N)$ and relative residual tolerance $\theta_N$ satisfying:
$$\theta_N\leq (1-\sqrt{2 \ve})/(1+\sqrt{2 \ve}) \leq (1-\sqrt{2 \beta_N(x_0^N,\tau_0^N)) L_N})/(1+\sqrt{2\beta_N(x_0^N,\tau_0^N) L_N}).$$
As shown above, Estimates \eqref{eq:unknown.NK1}-\eqref{eq:unknown.NK2} are satisfied with $\beta_N(x_0^N,\tau_0^N) L_N \leq \ve < 1/2$.  Theorem \ref{thm:inexactNK} then implies that the sequence $\{(x_k^N,\tau_k^N)\}_{k=0}^{\infty}$ generated from this inexact Newton procedure is well-defined and there exists $(x_*^N,\tau_*^N)$ which is the unique zero of $R_N$ in $\mc{B}((x_0^N,\tau_0^N),L_N^{-1})$ and the following estimates hold:
$$\|(x_*^N,\tau_*^N)-(x_0^N,T)\|\leq (1-\sqrt{1-2\beta_N(x_0^N,\tau_0^N) L_N})/L_N \leq 2 \beta_N(x_0^N,\tau_0^N),$$
\begin{align*}
\| & (x_{k+1}^N,\tau_{k+1}^N)  - (x_*^N,\tau_*^N)\| \\
&\leq \underbrace{\left[ \frac{(1+\theta_N)L_N}{2(1-\sqrt{2 \beta_N(x_0^N,\tau_0^N) L_N})}\right]}_{:= \hat D_{N,1}}\|(x_{k}^N,\tau_k^N)-(x_*^N,\tau_*^N)\|^2 \\
& + \theta_N\underbrace{\left[\frac{(1+\sqrt{2\beta_N(x_0^N,\tau_0^N) L_N})}{1-\sqrt{2 \beta_N(x_0^N,\tau_0^N) L_N}} \right]}_{:= \hat D_{N,2}}\|(x_k^N,\tau_k^N) - (x_*^N,\tau_*^N)\|.
\end{align*}
This proves Estimate \eqref{eq:unknown.2}.  It remains to prove Estimates \eqref{eq:unknown.1a}-\eqref{eq:unknown.1b}.  Repeating the above process with $(\alpha_N,T)$ as the initial guess in the inexact Newton process implies that there exists $(y_*^N,s_*^N) \in X^{2N+1} \times (0,\infty)$ with $R_N(y_*^N,s_*^N) = 0$ and: 
\begin{equation*}
\|(\alpha_N,T) - (y_*^N,s_*^N)\| \leq 2 \beta_N(\alpha_N,T) = 2 K_L (J_{1} + J_{\sigma})\hat L_2 (2\pi)^k(N+1)^{M_2 + \rho_2} K_p(N).
\end{equation*}
Estimate \eqref{eq:unknown.0} implies that there exists $N_3 \geq N_*$ so that if $N \geq N_3$, then:
\begin{equation}\label{eq:yNdef}
2 K_L (J_{1} + J_{\sigma})\hat L_2 (2\pi)^k(N+1)^{M_2 + \rho_2} K_p(N) \leq \hat L^{-1}_2 (N+1)^{-M_2 -\rho_2}/2 = L_N^{-1}/2.
\end{equation}
So, if $N \geq N_3$, then:
\begin{align*}
\|(y_*^N,s_*^N)  - (x_0^N,\tau_0^N)\| & \leq \|(y_*^N,s_*^N) - (\alpha_N,T)\| + \|(\alpha_N,T) - (x_0^N,\tau_0^N)\| && \text{(Triangle inequality)} \\
& \leq L_N^{-1}/2 + \|(\alpha_N,T) - (x_0^N,\tau_0^N)\| && \text{(Estimate \eqref{eq:yNdef})}\\
& \leq  L_N^{-1}/2 + \xi_N && \text{($\|(\alpha_N,T) - (x_0^N,\tau_0^N)\| \leq \xi_N$)} \\
& \leq L_N^{-1}/2 + L_N^{-1}/2 = L_N^{-1} && \text{(Estimate \eqref{eq:xnltnl})}
\end{align*}
Therefore $(y_*^N,s_*^N) \in \mc{B}((x_0^N,\tau_0^N),L_N^{-1})$ whenever $N \geq N_3$.  If $N \geq N_3$: then the fact that $R_N(y_*^N,s_*^N) = 0$ and $(y_*^N,\tau_*^N)$ is the unique zero of $R_N$ in $\mc{B}((x_0^N,\tau_0^N),L_N^{-1})$ implies that $(y_*^N,s_*^N) = (x_*^N,\tau_*^N)$ and therefore:
\begin{equation}\label{eq:unknown.lasta}
\|(x_*^N,\tau_*^N) - (\alpha_N,T) \| = \|(y_*^N,s_*^N) - (\alpha_N,T)\| \leq 2 K_L (J_{1}+J_{\sigma}) \hat L_2 (2\pi)^k (N+1)^{M_2 + \rho_2} K_p(N), \quad N \geq N_2.
\end{equation}
Consequently:
\begin{equation}\label{eq:unknown.lastb}
|\tau_*^N-T|, \|x_*^N - \alpha_N\|  \leq 2  K_L (J_{1}+J_{\sigma}) \hat L_2 (2\pi)^k (N+1)^{M_2 + \rho_2} K_p(N), \quad N \geq N_3.
\end{equation}
This proves Estimate \eqref{eq:unknown.1a} with $D_{k+1} = 2 K_L(J_1 + J_{\sigma}) \hat L_2 (2\pi)^k$.  Estimate \eqref{eq:unknown.1b} is proved as follows:
\begin{align*}
\|p^{(j)} - Q_N^{(j)}(x_*^N)\|_{L^2} & \leq \|p^{(j)} - Q_N^{(j)}(\alpha_N)\|_{L^2} + \|Q_N^{(j)}(\alpha_N) - Q_N^{(j)}(x_*^N)\|_{L^2} && \text{(Triangle inequality)} \\
& \leq  K_p(N) + \|Q_N^{(j)}(\alpha_N) - Q_N^{(j)}(x_*^N)\|_{L^2} && \text{(Estimate \eqref{eq:pfourierbound})} \\
& \leq K_p(N) + (2\pi N)^j\|x_0^N-\alpha_N\| && \text{(Lemma \ref{lem:Qlem1})}\\
& \leq  (1 + 2  K_L (J_{1}+J_{\sigma}) \hat L_2 (2\pi)^k (2\pi N)^j (N+1)^{M_2 + \rho_2})K_p(N) && \text{(Estimate \eqref{eq:unknown.lastb})} \\
& \leq (1 + 2 K_L (J_{1}+J_{\sigma}) \hat L_2 (2\pi)^{k+j}) (N+1)^{M_2 + \rho_2 + j} K_p(N).
 \end{align*}
 This proves Estimate \eqref{eq:unknown.1a} with $D_j = 1 + 2 K_L (J_{1}+J_{\sigma}) \hat L_2 (2\pi)^{k+j}$  for $j = 0,\hdots,k$.  This completes the proof.
 
\end{proof}
\end{comment}
